Time-Ordered Recent Event (TORE) Volumes for Event Cameras

Event cameras are an exciting, new sensor modality enabling high-speed imaging with extremely low-latency and wide dynamic range. Unfortunately, most machine learning architectures are not designed to directly handle sparse data, like that generated from event cameras. Many state-of-the-art algorithms for event cameras rely on interpolated event representations - obscuring crucial timing information, increasing the data volume, and limiting overall network performance. This paper details an event representation called Time-Ordered Recent Event (TORE) volumes. TORE volumes are designed to compactly store raw spike timing information with minimal information loss. This bio-inspired design is memory efficient, computationally fast, avoids time-blocking (i.e. fixed and predefined frame rates), and contains "local memory" from past data. The design is evaluated on a wide range of challenging tasks (e.g. event denoising, image reconstruction, classification, and human pose estimation) and is shown to dramatically improve state-of-the-art performance. TORE volumes are an easy-to-implement replacement for any algorithm currently utilizing event representations.

==> 4b_backupData.tex <==


\iffalse
\begin{table}
\centering
\caption{Image reconstruction scores for EV2VID and TORE on the Event Camera Dataset. Overall, EV2VID outperforms U-Net/TORE reconstruction.} 
\label{tab:imrecon}
\scalebox{1.0}{
\begin{tabular}{cccccc} 
\toprule
     & \multicolumn{2}{c}{(MSE)} & & \multicolumn{2}{c}{(SSIM)}            \\ 
\cline{2-3} \cline{5-6}
Dataset & EV2VID & TORE & & EV2VID & TORE\\ 
\hline\hline
boxes\_6dof & \textbf{0.04} & 0.05 & & \textbf{0.63} & 0.49\\
calibration & \textbf{0.04} & \textbf{0.04} & & \textbf{0.52} & 0.38\\
dynamic\_6dof & 0.08 & \textbf{0.07} & & \textbf{0.50} & \textbf{0.50}\\
office\_zigzag & \textbf{0.05} & \textbf{0.05} & & 0.50 & \textbf{0.51}\\
poster\_6dof & \textbf{0.04} & 0.05 & & \textbf{0.68} & 0.56\\
shapes\_6dof & \textbf{0.10} & 0.12 & & \textbf{0.44} & 0.29\\
slider\_depth & 0.06 & \textbf{0.04} & & \textbf{0.61} & 0.53\\
\bottomrule
mean & \textbf{0.06} & \textbf{0.06} & & \textbf{0.56} & 0.46\\
\bottomrule
\end{tabular}}
\end{table}
\fi

\iffalse
\begin{table*}
\centering
\caption{Scores for Image Reconstruction}
\label{tab:imrecon}
\scalebox{1.0}{
\begin{tabular}{cccccccc} 
\toprule
     & \multicolumn{3}{c}{(MSE)} & & \multicolumn{3}{c}{(SSIM)}            \\ 
\cline{2-4} \cline{6-8}
Dataset & EV2VID & TORE & TOREv2 & & EV2VID & TORE & TOREv2\\ 
\hline\hline
boxes\_6dof & \textbf{0.04} & 0.05 & 0.06 & & \textbf{0.63} & 0.49 & 0.51\\
calibration & 0.04 & 0.04 & \textbf{0.03} & & 0.52 & 0.38 & \textbf{0.58}\\
dynamic\_6dof & 0.08 & \textbf{0.07} & 0.13 & & \tetbf{0.50} & \textbf{0.50} & 0.38\\
office\_zigzag & \tetbf{0.05} & \textbf{0.05} & \textbf{0.05} & & 0.50 & \textbf{0.51} & 0.42\\
poster\_6dof & \textbf{0.04} & 0.05 & 0.09 & & \textbf{0.68} & 0.56 & 0.46\\
shapes\_6dof & 0.10 & 0.12 & \textbf{0.02} & & 0.44 & 0.29 & \textbf{0.71}\\
slider\_depth & 0.06 & \textbf{0.04} & 0.05 & & \textbf{0.61} & 0.53 & 0.52\\
\bottomrule
mean & 0.06 & 0.06 & \textbf{0.05} & & \textbf{0.56} & 0.46 & 0.51\\
\bottomrule
\end{tabular}}
\end{table*}
\fi

\iffalse\begin{table*}
\centering
\caption{Scores for Image Reconstruction}
\label{tab:imrecon}
\scalebox{1.0}{
\begin{tabular}{cccccccc} 
\toprule
     & \multicolumn{3}{c}{(MSE)} & & \multicolumn{3}{c}{(SSIM)}            \\ 
\cline{2-4} \cline{6-8}
Dataset & EV2VID & TORE & histeq & & EV2VID & TORE & histeq\\ 
\hline\hline
boxes\_6dof & 0.04 & 0.05 & 0.07 & & 0.63 & 0.49 & 0.46\\
calibration & 0.04 & 0.04 & 0.04 & & 0.52 & 0.38 & 0.38\\
dynamic\_6dof & 0.08 & 0.07 & 0.07 & & 0.50 & 0.50 & 0.56\\
office\_zigzag & 0.05 & 0.05 & 0.06 & & 0.50 & 0.51 & 0.54\\
poster\_6dof & 0.04 & 0.05 & 0.06 & & 0.68 & 0.56 & 0.55\\
shapes\_6dof & 0.10 & 0.12 & 0.06 & & 0.44 & 0.29 & 0.38\\
slider\_depth & 0.06 & 0.04 & 0.05 & & 0.61 & 0.53 & 0.53\\
\bottomrule
mean & 0.06 & 0.06 & 0.06 & & 0.56 & 0.46 & 0.49\\
\bottomrule
\end{tabular}}
\end{table*}
\fi


%transposed table
\begin{table*}[ht]
    \begin{center}
    \scalebox{0.5}{
\begin{tabular}{c|ccccccccccccccccccccccccccccccccc|c}
\hline
\multicolumn{1}{c|}{}                                                                          & \multicolumn{33}{c|}{3D MPJPE (mm) per Movement} & Overall         \\
\multicolumn{1}{c|}{Method} & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & Mean (mm)           \\ \hline
\multicolumn{1}{c|}{DHP19} & 112.8 & 98.5 & 84.6 & 77.6 & 103.2 & 120.3 & 74.5 & 71.9 & 53.6 & 68.9 & 74.2 & 51.4 & 54.8 & 52.3 & 144.8 & 130.4 & 107.1 & 134.2 & 100.6 & 89.5 & 54.8 & 74.8 & 109.4 & 109.1 & 115.4 & 105.7 & 91.2 & 94.0 & 107.8 & 108.1 & 111.0 & 119.8 & 124.5 & 94.8\\
\multicolumn{1}{c|}{TORE} & 59.6 & 53.0 & 65.5 & 63.0 & 63.6 & 67.7 & 46.3 & 48.5 & 43.1 & 53.0 & 52.8 & 46.5 & 47.2 & 44.5 & 76.2 & 71.3 & 71.3 & 75.0 & 67.4 & 62.0 & 48.7 & 58.7 & 62.1 & 64.1 & 73.6 & 69.5 & 55.0 & 48.8 & 52.4 & 50.8 & 49.7 & 58.5 & 55.5 & 58.4\\
\hline
\end{tabular}
}
    \end{center}
    \caption{3D pose reconstruction error for the DHP19 dataset. The table presents MPJPE (mm) for the five test subjects (Sub13 to Sub17) on all 33 movements (Mov). The final column is reported results from the prior SOTA on the DHP19~\cite{calabrese2019dhp19}.}
    \label{tb:MPJPE}
\end{table*}


\iffalse
\begin{table}
\centering
\caption{Test set 2D MPJPE (pixel) for the CNN, trained on the two frontal camera views (camera 2 and 3). In bold the selected confidence threshold (Conf. thr.) for 3D projection.}
\label{tab:2DMPJPE}
\scalebox{0.98}{
\begin{tabular}{cccccccc} 
\toprule
     &     & \multicolumn{6}{c}{Threshold}            \\ 
\cline{3-8}
Feat & Cam & 0    & 0.1  & 0.2  & 0.3  & 0.4  & 0.5   \\ 
\hline\hline
CCF & 2 & 7.72 & 7.45 & 7.25 & 7.18 & 7.27 & 7.47  \\
CCF & 3 & 7.61 & 7.13 & 6.92 & 6.87 & 6.88 & 7.11  \\
MPF & 2 & 5.36 & 5.18 & 5.17 & 5.16 & 5.15 & 5.15  \\
MPF & 3 & 5.67 & 5.52 & 5.52 & 5.55 & 5.62 & 5.65  \\
\bottomrule
\end{tabular}}
\end{table}
\fi


\iffalse
\begin{table}[ht]
    \begin{center}
    \scalebox{0.8}{
\begin{tabular}{cc|ccccc|c}
\hline
\multicolumn{1}{c|}{}                                                                          &    & \multicolumn{5}{c|}{Testing Subject Number} & Mean          \\
\multicolumn{1}{c|}{Se}                                                                        & M  & Sub13   & Sub14  & Sub15  & Sub16  & Sub17  & M             \\ \hline
\multicolumn{1}{c|}{\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}1\\ Mean\\ 109\end{tabular}}}   & 1  & 58.4    & 381.39 & 52.95  & 122.09 & 122.78 & 147.5         \\
\multicolumn{1}{c|}{}                                                                          & 2  & 67.33   & 70.79  & 74.14  & 102.55 & 159.38 & 94.8          \\
\multicolumn{1}{c|}{}                                                                          & 3  & 78.54   & 231.58 & 91.39  & 97.77  & 167.56 & 133.4         \\
\multicolumn{1}{c|}{}                                                                          & 4  & 63.32   & 226.51 & 59.31  & 116.48 & 112.28 & 115.6         \\
\multicolumn{1}{c|}{}                                                                          & 5  & 64.64   & 53.8   & 54.89  & 78.08  & 139.38 & 78.2          \\
\multicolumn{1}{c|}{}                                                                          & 6  & 51.96   & 127.77 & 89.63  & 90.36  & 196.64 & 111.3         \\
\multicolumn{1}{c|}{}                                                                          & 7  & 70.08   & 81.52  & 107.93 & 135.09 & 193.61 & 117.6         \\
\multicolumn{1}{c|}{}                                                                          & 8  & 59.21   & 63.26  & 57.63  & 75.02  & 113    & 73.6          \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}2\\ Mean\\ 81.3\end{tabular}}}  & 9  & 37.95   & 66.66  & 54.45  & 72.56  & 112.32 & 68.8          \\
\multicolumn{1}{c|}{}                                                                          & 10 & 66.01   & 61.42  & 67.25  & 105.23 & 181.28 & 96.2          \\
\multicolumn{1}{c|}{}                                                                          & 11 & 72.13   & 77.27  & 75.52  & 90.95  & 126.99 & 88.6          \\
\multicolumn{1}{c|}{}                                                                          & 12 & 55.01   & 69.24  & 74.98  & 101.09 & 120.64 & 84.2          \\
\multicolumn{1}{c|}{}                                                                          & 13 & 67.66   & 80.87  & 75.79  & 95.83  & 86.88  & 81.4          \\
\multicolumn{1}{c|}{}                                                                          & 14 & 53.08   & 79.26  & 55.89  & 73.16  & 81.57  & 68.6          \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}3\\ Mean\\ 109.3\end{tabular}}} & 15 & 73.95   & 192.75 & 74.61  & 127.79 & 132.88 & 120.4         \\
\multicolumn{1}{c|}{}                                                                          & 16 & 52      & 318.88 & 66.53  & 142.07 & 135.53 & 143           \\
\multicolumn{1}{c|}{}                                                                          & 17 & 66.61   & 141.33 & 59.4   & 100.17 & 93.73  & 92.2          \\
\multicolumn{1}{c|}{}                                                                          & 18 & 60.34   & 99.86  & 56.48  & 121.66 & 122.24 & 92.1          \\
\multicolumn{1}{c|}{}                                                                          & 19 & 78.23   & 122.91 & 51.63  & 136.21 & 136.54 & 105.1         \\
\multicolumn{1}{c|}{}                                                                          & 20 & 51.72   & 122.64 & 54.04  & 128.23 & 158.43 & 103           \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}4\\ Mean\\ 100.5\end{tabular}}} & 21 & 46.2    & 72.6   & 90.15  & 80.65  & 96.76  & 77.3          \\
\multicolumn{1}{c|}{}                                                                          & 22 & 74.13   & 87.66  & 77.26  & 125.49 & 123.69 & 97.6          \\
\multicolumn{1}{c|}{}                                                                          & 23 & 81.63   & nan    & 85.59  & 84.7   & 134.35 & 96.6          \\
\multicolumn{1}{c|}{}                                                                          & 24 & 60.57   & nan    & 126.74 & 76.83  & 170.08 & 108.6         \\
\multicolumn{1}{c|}{}                                                                          & 25 & 133.13  & nan    & 133.47 & 125.3  & 141.15 & 133.3         \\
\multicolumn{1}{c|}{}                                                                          & 26 & 69.13   & nan    & 115.12 & 95.07  & 105.98 & 96.3          \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}5\\ Mean\\ 79.3\end{tabular}}}  & 27 & 49.94   & 104.78 & 43.76  & 76.41  & 86.19  & 72.2          \\
\multicolumn{1}{c|}{}                                                                          & 28 & 38.44   & 60.25  & 45.49  & 103.78 & 122.36 & 74.1          \\
\multicolumn{1}{c|}{}                                                                          & 29 & 44.18   & nan    & 53.32  & 113.87 & 96.95  & 77.1          \\
\multicolumn{1}{c|}{}                                                                          & 30 & 62.52   & 72.45  & 63.57  & 82.94  & 138.73 & 84            \\
\multicolumn{1}{c|}{}                                                                          & 31 & 56.15   & 55.18  & 55.73  & 94.36  & 86.13  & 69.5          \\
\multicolumn{1}{c|}{}                                                                          & 32 & 57.96   & 90.22  & 71.42  & 68.71  & 140.06 & 85.7          \\
\multicolumn{1}{c|}{}                                                                          & 33 & 50.57   & 66     & 119.98 & 110.31 & 112.05 & 91.8          \\ \hline
\multicolumn{2}{c}{Mean}                                                                            & 62.8    & 117.1  & 73.8   & 101.5  & 128.7  & \textbf{96.2} \\ \hline
\end{tabular}
}
    \end{center}
    \caption{(v0???) One cam2 event camera testing results on the 5 test subjects (Sub13 to Sub17) on the 33 movements (M), over separate subjects (S) and whole sessions (Se). The evaluation is performed on DHP19 under $Protocol \#1$ with MPJPE (mm).}
    \label{tb:MPJPE}
\end{table}
\fi

\iffalse
\begin{table}[ht]
    \begin{center}
    \scalebox{0.8}{
\begin{tabular}{cc|ccccc|c}
\hline
\multicolumn{1}{c|}{}                                                                         &    & \multicolumn{5}{c|}{Testing Subject Number} & Mean          \\
\multicolumn{1}{c|}{Se}                                                                       & M  & Sub13  & Sub14   & Sub15  & Sub16  & Sub17  & M             \\ \hline
\multicolumn{1}{c|}{\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}1\\ Mean\\ 72.4\end{tabular}}} & 1  & 34.41  & 469.7   & 38.17  & 58.49  & 84.52  & 137.1         \\
\multicolumn{1}{c|}{}                                                                         & 2  & 28.29  & 45.57   & 41.24  & 62.25  & 85.85  & 52.6          \\
\multicolumn{1}{c|}{}                                                                         & 3  & 39.38  & 89.59   & 47.14  & 60.16  & 67.72  & 60.8          \\
\multicolumn{1}{c|}{}                                                                         & 4  & 49.82  & 109.8   & 47.51  & 71.05  & 67.07  & 69.1          \\
\multicolumn{1}{c|}{}                                                                         & 5  & 52.59  & 70.63   & 47.63  & 71.54  & 69.96  & 62.5          \\
\multicolumn{1}{c|}{}                                                                         & 6  & 51.21  & 164.51  & 68.48  & 71.48  & 95.43  & 90.2          \\
\multicolumn{1}{c|}{}                                                                         & 7  & 32.22  & 55.28   & 52.35  & 64.96  & 69.99  & 55            \\
\multicolumn{1}{c|}{}                                                                         & 8  & 29.48  & 60.24   & 47.06  & 60.78  & 63.57  & 52.2          \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}2\\ Mean\\ 55.5\end{tabular}}} & 9  & 24.66  & 54.14   & 37.51  & 70.57  & 54.7   & 48.3          \\
\multicolumn{1}{c|}{}                                                                         & 10 & 36.54  & 56.83   & 39.92  & 74.97  & 119.63 & 65.6          \\
\multicolumn{1}{c|}{}                                                                         & 11 & 43.12  & 49.12   & 45.54  & 74.52  & 77.55  & 58            \\
\multicolumn{1}{c|}{}                                                                         & 12 & 23.64  & 57.86   & 38.9   & 84.18  & 62.65  & 53.4          \\
\multicolumn{1}{c|}{}                                                                         & 13 & 38.07  & 53.16   & 48.59  & 77.81  & 57.2   & 55            \\
\multicolumn{1}{c|}{}                                                                         & 14 & 29.64  & 58.68   & 43.82  & 72.3   & 58.95  & 52.7          \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}3\\ Mean\\ 72.9\end{tabular}}} & 15 & 56.55  & 150.79  & 55.17  & 99.87  & 72.12  & 86.9          \\
\multicolumn{1}{c|}{}                                                                         & 16 & 55.63  & 149.81  & 43.76  & 95.8   & 65.03  & 82            \\
\multicolumn{1}{c|}{}                                                                         & 17 & 36.83  & 129.45  & 42.51  & 79.31  & 62.51  & 70.1          \\
\multicolumn{1}{c|}{}                                                                         & 18 & 33.55  & 97.43   & 49.46  & 80.48  & 64.3   & 65            \\
\multicolumn{1}{c|}{}                                                                         & 19 & 41.53  & 108.66  & 43.47  & 82.11  & 65.2   & 68.2          \\
\multicolumn{1}{c|}{}                                                                         & 20 & 37.97  & 96.28   & 41.08  & 78.57  & 71.6   & 65.1          \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}4\\ Mean\\ 66.8\end{tabular}}} & 21 & 31.82  & 57.83   & 48.41  & 76.65  & 63.57  & 55.7          \\
\multicolumn{1}{c|}{}                                                                         & 22 & 74.59  & 84.26   & 51.66  & 85.27  & 65.69  & 72.3          \\
\multicolumn{1}{c|}{}                                                                         & 23 & 31.53  & nan     & 63.87  & 68.71  & 81.79  & 61.5          \\
\multicolumn{1}{c|}{}                                                                         & 24 & 33.65  & nan     & 88.21  & 72.32  & 74.83  & 67.3          \\
\multicolumn{1}{c|}{}                                                                         & 25 & 51.22  & nan     & 93.69  & 71.25  & 76.49  & 73.2          \\
\multicolumn{1}{c|}{}                                                                         & 26 & 43.74  & nan     & 78.66  & 74.49  & 93.16  & 72.5          \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}5\\ Mean\\ 79.3\end{tabular}}} & 27 & 30.52  & 88.75   & 37.88  & 70.46  & 52.35  & 56            \\
\multicolumn{1}{c|}{}                                                                         & 28 & 29.12  & 43.83   & 37.5   & 67.65  & 56.47  & 46.9          \\
\multicolumn{1}{c|}{}                                                                         & 29 & 27.67  & nan     & 42.68  & 74.49  & 56.21  & 50.3          \\
\multicolumn{1}{c|}{}                                                                         & 30 & 32.48  & 53.87   & 53.19  & 73.68  & 57.09  & 54.1          \\
\multicolumn{1}{c|}{}                                                                         & 31 & 34.92  & 52.9    & 38.12  & 69.55  & 60.95  & 51.3          \\
\multicolumn{1}{c|}{}                                                                         & 32 & 38.54  & 88.11   & 57.99  & 63.99  & 57.49  & 61.2          \\
\multicolumn{1}{c|}{}                                                                         & 33 & 35.22  & 60.27   & 82.99  & 76.33  & 56.83  & 62.3          \\ \hline
\multicolumn{2}{c}{Mean}                                                                           & 38.5   & 94.9    & 51.3   & 73.8   & 69.3   & \textbf{64.7} \\ \hline
\end{tabular}
}
    \end{center}
    \caption{(4CAM EXP v1) Two event camera testing results on the 5 test subjects (Sub13 to Sub17) on the 33 movements (M), over separate subjects (S) and whole sessions (Se). The evaluation is performed on DHP19 under $Protocol \#1$ with MPJPE (mm).}
    \label{tb:MPJPE_two_event}
\end{table}

\begin{table}[ht]
    \begin{center}
    \scalebox{0.8}{
\begin{tabular}{cc|ccccc|c}
\hline
\multicolumn{1}{c|}{}                                                                         &    & \multicolumn{5}{c|}{Testing Subject Number} & Mean          \\
\multicolumn{1}{c|}{Se}                                                                       & M  & Sub13  & Sub14   & Sub15  & Sub16  & Sub17  & M             \\ \hline
\multicolumn{1}{c|}{\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}1\\ Mean\\ 55\end{tabular}}}   & 1  & 28.82  & 42.49   & 36.26  & 75.88  & 86.19  & 53.9          \\
\multicolumn{1}{c|}{}                                                                         & 2  & 24.96  & 39.88   & 36.46  & 74.92  & 93.24  & 53.9          \\
\multicolumn{1}{c|}{}                                                                         & 3  & 28.47  & 102.22  & 43.86  & 60.82  & 67.53  & 60.6          \\
\multicolumn{1}{c|}{}                                                                         & 4  & 32.34  & 108.48  & 41.71  & 68.51  & 69.42  & 64.1          \\
\multicolumn{1}{c|}{}                                                                         & 5  & 29.41  & 51.23   & 40.97  & 80.27  & 74.69  & 55.3          \\
\multicolumn{1}{c|}{}                                                                         & 6  & 40.1   & 46.89   & 38.91  & 71.63  & 86.36  & 56.8          \\
\multicolumn{1}{c|}{}                                                                         & 7  & 24.62  & 52.65   & 37.51  & 64.5   & 62.16  & 48.3          \\
\multicolumn{1}{c|}{}                                                                         & 8  & 23.18  & 49.28   & 41.05  & 61.32  & 60.31  & 47            \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}2\\ Mean\\ 49.5\end{tabular}}} & 9  & 20.41  & 43.78   & 29.36  & 67.64  & 53.68  & 43            \\
\multicolumn{1}{c|}{}                                                                         & 10 & 27.13  & 45.5    & 36.04  & 69.16  & 97.82  & 55.1          \\
\multicolumn{1}{c|}{}                                                                         & 11 & 40.23  & 54.06   & 38.19  & 69.95  & 77.08  & 55.9          \\
\multicolumn{1}{c|}{}                                                                         & 12 & 20.24  & 49.91   & 34.28  & 73.52  & 58.38  & 47.3          \\
\multicolumn{1}{c|}{}                                                                         & 13 & 32.55  & 46.92   & 38.27  & 70.08  & 56.48  & 48.9          \\
\multicolumn{1}{c|}{}                                                                         & 14 & 22.27  & 46.91   & 40.1   & 66.34  & 59.24  & 47            \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}3\\ Mean\\ 70.9\end{tabular}}} & 15 & 28.62  & 121.65  & 45.06  & 85.06  & 81.92  & 72.5          \\
\multicolumn{1}{c|}{}                                                                         & 16 & 36.81  & 115.77  & 40.56  & 86.7   & 72.7   & 70.5          \\
\multicolumn{1}{c|}{}                                                                         & 17 & 33.16  & 144.56  & 36.62  & 79.98  & 67.93  & 72.5          \\
\multicolumn{1}{c|}{}                                                                         & 18 & 97.25  & 103.59  & 40.84  & 72.56  & 79.11  & 78.7          \\
\multicolumn{1}{c|}{}                                                                         & 19 & 29.75  & 102.06  & 37.61  & 79.77  & 75.27  & 64.9          \\
\multicolumn{1}{c|}{}                                                                         & 20 & 32.32  & 132.33  & 31.28  & 70.9   & 65.86  & 66.5          \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}4\\ Mean\\ 61.1\end{tabular}}} & 21 & 26.66  & 50.72   & 43.58  & 71.99  & 58.83  & 50.4          \\
\multicolumn{1}{c|}{}                                                                         & 22 & 53.77  & 66.92   & 46.1   & 74.33  & 63.32  & 60.9          \\
\multicolumn{1}{c|}{}                                                                         & 23 & 30.32  & 72.05   & 62.02  & 66.6   & 81.3   & 62.5          \\
\multicolumn{1}{c|}{}                                                                         & 24 & 25.12  & 59.9    & 66.41  & 70.83  & 75.28  & 59.5          \\
\multicolumn{1}{c|}{}                                                                         & 25 & 50.69  & 66.51   & 85.68  & 64.6   & 80.03  & 69.5          \\
\multicolumn{1}{c|}{}                                                                         & 26 & 35.26  & 54.6    & 74.7   & 69.97  & 85.34  & 64            \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}5\\ Mean\\ 53.2\end{tabular}}} & 27 & 27.2   & 92.41   & 31.8   & 69.91  & 59.97  & 56.3          \\
\multicolumn{1}{c|}{}                                                                         & 28 & 32.62  & 43.16   & 35.66  & 70.15  & 68.5   & 50            \\
\multicolumn{1}{c|}{}                                                                         & 29 & 27.39  & nan     & 34.88  & 77.45  & 64.43  & 51            \\
\multicolumn{1}{c|}{}                                                                         & 30 & 31.25  & 44.52   & 37.3   & 69.68  & 69.85  & 50.5          \\
\multicolumn{1}{c|}{}                                                                         & 31 & 31.02  & 52.75   & 35.66  & 74.89  & 68.55  & 52.6          \\
\multicolumn{1}{c|}{}                                                                         & 32 & 27.39  & 91.66   & 36.2   & 66.75  & 71.33  & 58.7          \\
\multicolumn{1}{c|}{}                                                                         & 33 & 29.24  & 48.61   & 47.27  & 77.53  & 60.98  & 52.7          \\ \hline
\multicolumn{2}{c}{Mean}                                                                           & 32.7   & 70.1    & 42.5   & 71.9   & 71.3   & \textbf{57.6} \\ \hline
\end{tabular}
}
    \end{center}
    \caption{(4cam exp v2) Four event camera testing results(using exp0 exp1 exp2 and exp3) on the 5 test subjects (Sub13 to Sub17) on the 33 movements (M), over separate subjects (S) and whole sessions (Se). The evaluation is performed on DHP19 under $Protocol \#1$ with MPJPE (mm).}
    \label{tb:MPJPE_four_event}
\end{table}



\begin{table}[ht]
    \begin{center}
    \scalebox{0.8}{
\begin{tabular}{cc|ccccc|c}
\hline
\multicolumn{1}{c|}{}                                                                         &    & \multicolumn{5}{c|}{Testing Subject Number} & Mean          \\
\multicolumn{1}{c|}{Se}                                                                       & M  & Sub13  & Sub14   & Sub15  & Sub16  & Sub17  & M             \\ \hline
\multicolumn{1}{c|}{\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}1\\ Mean\\ 58.3\end{tabular}}} & 1  & 28.11  & 38.18   & 40.04  & 62.34  & 125.69 & 58.9          \\
\multicolumn{1}{c|}{}                                                                         & 2  & 24.25  & 35.98   & 42.76  & 65.53  & 96.18  & 52.9          \\
\multicolumn{1}{c|}{}                                                                         & 3  & 30.36  & 100.92  & 41.76  & 61.08  & 64.53  & 59.7          \\
\multicolumn{1}{c|}{}                                                                         & 4  & 31.35  & 118.92  & 46.22  & 68.27  & 102.48 & 73.4          \\
\multicolumn{1}{c|}{}                                                                         & 5  & 30.79  & 43.18   & 45.75  & 85.41  & 109.28 & 62.9          \\
\multicolumn{1}{c|}{}                                                                         & 6  & 31.8   & 52.04   & 40.88  & 104.17 & 80.38  & 61.9          \\
\multicolumn{1}{c|}{}                                                                         & 7  & 24.31  & 43.91   & 40.16  & 63.2   & 64.46  & 47.2          \\
\multicolumn{1}{c|}{}                                                                         & 8  & 27.46  & 50.63   & 43.85  & 59.74  & 65.89  & 49.5          \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}2\\ Mean\\ 48.5\end{tabular}}} & 9  & 22.09  & 47.56   & 33.17  & 63.79  & 53.71  & 44.1          \\
\multicolumn{1}{c|}{}                                                                         & 10 & 28.33  & 45.33   & 37.02  & 62.92  & 92.42  & 53.2          \\
\multicolumn{1}{c|}{}                                                                         & 11 & 37.61  & 43.6    & 39.21  & 67.93  & 75.85  & 52.8          \\
\multicolumn{1}{c|}{}                                                                         & 12 & 20.73  & 52.96   & 36.27  & 69.34  & 57.77  & 47.4          \\
\multicolumn{1}{c|}{}                                                                         & 13 & 35.09  & 45.38   & 40.26  & 62.5   & 54.85  & 47.6          \\
\multicolumn{1}{c|}{}                                                                         & 14 & 23.01  & 48.13   & 39.08  & 61.91  & 57.55  & 45.9          \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}3\\ Mean\\ 69.8\end{tabular}}} & 15 & 27.76  & 151.67  & 51.76  & 85.96  & 66.53  & 76.7          \\
\multicolumn{1}{c|}{}                                                                         & 16 & 31.57  & 93.87   & 39.69  & 88.78  & 70.08  & 64.8          \\
\multicolumn{1}{c|}{}                                                                         & 17 & 37.52  & 137.71  & 43.4   & 77.18  & 64.71  & 72.1          \\
\multicolumn{1}{c|}{}                                                                         & 18 & 46.42  & 125.1   & 47.16  & 82.43  & 71.63  & 74.5          \\
\multicolumn{1}{c|}{}                                                                         & 19 & 27.73  & 113.73  & 42.89  & 78.18  & 76.56  & 67.8          \\
\multicolumn{1}{c|}{}                                                                         & 20 & 31.72  & 99.78   & 40.14  & 79.74  & 63.59  & 63            \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}4\\ Mean\\ 62.4\end{tabular}}} & 21 & 25.99  & 50.95   & 46.68  & 67.53  & 58.65  & 50            \\
\multicolumn{1}{c|}{}                                                                         & 22 & 50.3   & 54.85   & 46.99  & 68.47  & 63.95  & 56.9          \\
\multicolumn{1}{c|}{}                                                                         & 23 & 36.29  & 78.54   & 65.68  & 62.44  & 64.26  & 61.4          \\
\multicolumn{1}{c|}{}                                                                         & 24 & 34.63  & 62.8    & 85.95  & 65.51  & 74.27  & 64.6          \\
\multicolumn{1}{c|}{}                                                                         & 25 & 46.56  & 75.46   & 95.01  & 62.63  & 89.29  & 73.8          \\
\multicolumn{1}{c|}{}                                                                         & 26 & 37.78  & 57.26   & 72.33  & 71.13  & 99.6   & 67.6          \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}5\\ Mean\\ 53.2\end{tabular}}} & 27 & 28.82  & 90.32   & 38.19  & 61.62  & 57.98  & 55.4          \\
\multicolumn{1}{c|}{}                                                                         & 28 & 27.29  & 46.75   & 38.94  & 70.32  & 64.18  & 49.5          \\
\multicolumn{1}{c|}{}                                                                         & 29 & 32.41  & nan     & 39.06  & 68.87  & 73.39  & 53.4          \\
\multicolumn{1}{c|}{}                                                                         & 30 & 30.78  & 47.04   & 39.34  & 70.1   & 67.85  & 51            \\
\multicolumn{1}{c|}{}                                                                         & 31 & 36.86  & 41.65   & 39.26  & 67.14  & 67.84  & 50.6          \\
\multicolumn{1}{c|}{}                                                                         & 32 & 28.22  & 93.82   & 38.9   & 70.66  & 65.32  & 59.4          \\
\multicolumn{1}{c|}{}                                                                         & 33 & 26.65  & 50.44   & 58.9   & 81.28  & 65.77  & 56.6          \\ \hline
\multicolumn{2}{c}{Mean}                                                                           & 31.5   & 70      & 46.6   & 70.9   & 73.5   & \textbf{58.4} \\ \hline
\end{tabular}
}
    \end{center}
    \caption{(2CAM hist23 hist threshold 10) Two event camera testing results on the 5 test subjects (Sub13 to Sub17) on the 33 movements (M), over separate subjects (S) and whole sessions (Se). The evaluation is performed on DHP19 under $Protocol \#1$ with MPJPE (mm).}
    \label{tb:MPJPE_two_event}
\end{table}

\begin{table}[ht]
    \begin{center}
    \scalebox{0.8}{
\begin{tabular}{cc|ccccc|c}
\hline
\multicolumn{1}{c|}{}                                                                         &    & \multicolumn{5}{c|}{Testing Subject Number} & Mean          \\
\multicolumn{1}{c|}{Se}                                                                       & M  & Sub13  & Sub14   & Sub15  & Sub16  & Sub17  & M             \\ \hline
\multicolumn{1}{c|}{\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}1\\ Mean\\ 56.9\end{tabular}}} & 1  & 29.07  & 39.58   & 33.2   & 60.75  & 111.86 & 54.9          \\
\multicolumn{1}{c|}{}                                                                         & 2  & 27.27  & 37.74   & 38.6   & 66.17  & 105.72 & 55.1          \\
\multicolumn{1}{c|}{}                                                                         & 3  & 28.25  & 133.77  & 38.19  & 58.5   & 65.54  & 64.8          \\
\multicolumn{1}{c|}{}                                                                         & 4  & 30.97  & 113.54  & 44.9   & 64.76  & 70.24  & 64.9          \\
\multicolumn{1}{c|}{}                                                                         & 5  & 30.28  & 47.06   & 38.16  & 87.73  & 100.81 & 60.8          \\
\multicolumn{1}{c|}{}                                                                         & 6  & 29.65  & 47.45   & 38     & 101.51 & 87.6   & 60.8          \\
\multicolumn{1}{c|}{}                                                                         & 7  & 25.61  & 42.14   & 38.18  & 62.59  & 63.31  & 46.4          \\
\multicolumn{1}{c|}{}                                                                         & 8  & 24.53  & 44.43   & 41.64  & 62.43  & 65.82  & 47.8          \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}2\\ Mean\\ 47.1\end{tabular}}} & 9  & 21.78  & 42.95   & 29.08  & 61.89  & 53.54  & 41.8          \\
\multicolumn{1}{c|}{}                                                                         & 10 & 26.31  & 39.35   & 35.03  & 63.42  & 92.53  & 51.3          \\
\multicolumn{1}{c|}{}                                                                         & 11 & 38.54  & 47.8    & 34.66  & 67.92  & 76.49  & 53.1          \\
\multicolumn{1}{c|}{}                                                                         & 12 & 19.83  & 46.89   & 33.5   & 67.72  & 57.96  & 45.2          \\
\multicolumn{1}{c|}{}                                                                         & 13 & 32.42  & 44.56   & 37.02  & 60.83  & 54.76  & 45.9          \\
\multicolumn{1}{c|}{}                                                                         & 14 & 20.59  & 47.21   & 37.69  & 61.25  & 58.54  & 45.1          \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}3\\ Mean\\ 67.2\end{tabular}}} & 15 & 26.59  & 139.63  & 46.74  & 83.46  & 69.65  & 73.2          \\
\multicolumn{1}{c|}{}                                                                         & 16 & 29.85  & 113.64  & 36.65  & 88.33  & 68.49  & 67.4          \\
\multicolumn{1}{c|}{}                                                                         & 17 & 31.87  & 131.24  & 42.54  & 75.52  & 67.96  & 69.8          \\
\multicolumn{1}{c|}{}                                                                         & 18 & 39.02  & 101.89  & 45.19  & 80.72  & 74.97  & 68.4          \\
\multicolumn{1}{c|}{}                                                                         & 19 & 26.88  & 104.2   & 38.22  & 74.51  & 78.14  & 64.4          \\
\multicolumn{1}{c|}{}                                                                         & 20 & 29.12  & 92.56   & 37.79  & 76.19  & 65.64  & 60.3          \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}4\\ Mean\\ 62.2\end{tabular}}} & 21 & 24.58  & 47.9    & 43.51  & 66.15  & 57.76  & 48            \\
\multicolumn{1}{c|}{}                                                                         & 22 & 46.74  & 54.09   & 47.11  & 71.36  & 63.15  & 56.5          \\
\multicolumn{1}{c|}{}                                                                         & 23 & 31.07  & 88.01   & 67.96  & 61.26  & 65.48  & 62.8          \\
\multicolumn{1}{c|}{}                                                                         & 24 & 34.05  & 63.14   & 93.59  & 68     & 74.55  & 66.7          \\
\multicolumn{1}{c|}{}                                                                         & 25 & 43.72  & 75.44   & 94.78  & 60.51  & 86.37  & 72.2          \\
\multicolumn{1}{c|}{}                                                                         & 26 & 35.7   & 56.94   & 71.87  & 70.06  & 99.7   & 66.9          \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}5\\ Mean\\ 51.9\end{tabular}}} & 27 & 25.5   & 91.25   & 32.78  & 66.01  & 58.08  & 54.7          \\
\multicolumn{1}{c|}{}                                                                         & 28 & 24.48  & 44.98   & 35.47  & 69.88  & 62.56  & 47.5          \\
\multicolumn{1}{c|}{}                                                                         & 29 & 26.59  & nan     & 32.15  & 67.93  & 68.61  & 48.8          \\
\multicolumn{1}{c|}{}                                                                         & 30 & 29.59  & 46.09   & 35.35  & 71.05  & 63.37  & 49.1          \\
\multicolumn{1}{c|}{}                                                                         & 31 & 35.19  & 48.7    & 33.15  & 68.41  & 64.84  & 50.1          \\
\multicolumn{1}{c|}{}                                                                         & 32 & 29.41  & 88.7    & 34.26  & 72.49  & 62.38  & 57.4          \\
\multicolumn{1}{c|}{}                                                                         & 33 & 28.67  & 55.25   & 49.07  & 77.83  & 62.82  & 54.7          \\ \hline
\multicolumn{2}{c}{Mean}                                                                           & 29.8   & 69.3    & 43.5   & 70.2   & 72.1   & \textbf{56.9} \\ \hline
\end{tabular}
}
    \end{center}
    \caption{(4cam hist threshold 10) Four event camera testing results(using exp0 exp1 exp2 and exp3) on the 5 test subjects (Sub13 to Sub17) on the 33 movements (M), over separate subjects (S) and whole sessions (Se). The evaluation is performed on DHP19 under $Protocol \#1$ with MPJPE (mm).}
    \label{tb:MPJPE_four_event}
\end{table}
\fi

% \begin{table}[ht]
%     \begin{center}
%     \scalebox{0.8}{
    
%     table to here
    
    
%     }
%     \end{center}
%     \caption{ The evaluation is performed on DHP19 under $Protocol \#1$ with MPJPE (mm).}
%     \label{tb:MPJPE_two_event}
% \end{table}


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

